LO2: Microservice API Anomaly Dataset of Logs and Metrics

Context. Microservice-based systems have gained significant attention over the past years. A critical factor for understanding and analyzing the behavior of these systems is the collection of monitoring data such as logs, metrics, and traces. These data modalities can be used for anomaly detection and root cause analysis of failures. In particular, multi-modal methods utilizing several types of this data at once have gained traction in the research community since these three modalities capture different dimensions of system behavior. Aim. We provide a dataset that supports research on anomaly detection and architectural degradation in microservice systems. We generate a comprehensive dataset of logs, metrics, and traces from a production microservice system to enable the exploration of multi-modal fusion methods that integrate multiple data modalities. Method. We dynamically tested the various APIs of the MS-based system, implementing the OAuth2.0 protocol using the Locust tool. For each execution of the prepared test suite, we collect logs and performance metrics for correct and erroneous calls with data labeled according to the error triggered during the call. Contributions. We collected approximately 657,000 individual log files, totaling over two billion log lines. In addition, we collected more than 45 million individual metric files that contain 485 unique metrics. We provide an initial analysis of logs, identify key metrics through PCA, and discuss challenges in collecting traces for this system. Moreover, we highlight the possibilities for making a more fine-grained version of the data set. This work advances anomaly detection in microservice systems using multiple data sources.

==> Tables/loganalysis_short.tex <==
\begin{table}[ht]
\centering
\caption{Anomaly Detection on Each Service Log}
\label{tab:logs}
\begin{tabular}{l p{0.62cm} p{0.62cm} p{0.62cm} p{0.7cm} p{0.62cm} p{0.62cm} p{0.62cm}}
\hline
\textbf{Log Name:} & Client & Code & Key & Ref-t. & Service & Token & User \\ 
\hline
\multicolumn{8}{l}{\textbf{Model and Score:} DecisionTree F1 Score} \\ 
\hline
\textbf{Average} & 0.951 & 0.476 & 0.353 & 0.545 & 0.842 & 0.980 & 0.663 \\ 
\textbf{Min}     & 0.649 & 0.000 & 0.034 & 0.281 & 0.673 & 0.935 & 0.396 \\ 
\textbf{Max}     & 1.000 & 1.000 & 0.667 & 1.000 & 1.000 & 1.000 & 1.000 \\ 
\hline
\multicolumn{8}{l}{\textbf{Model and Score:} KMeans AUCROC} \\ 
\hline
\textbf{Average} & 0.797 & 0.843 & 0.727 & 0.849 & 0.531 & 0.978 & 0.597 \\ 
\textbf{Min}     & 0.678 & 0.754 & 0.517 & 0.756 & 0.385 & 0.925 & 0.392 \\ 
\textbf{Max}     & 0.991 & 1.000 & 0.887 & 1.000 & 0.998 & 1.000 & 1.000 \\
\hline
\end{tabular}
\end{table}


==> Tables/services_long.tex <==
%% This is the original table, a shorter version is in services_short.tex
\begin{table}
\renewcommand{\arraystretch}{1.5} 
\caption{List of Services of Light-OAuth2 System and Implemented Locust Tasks}
\label{tab:services_long}
\centering
\begin{tabular}{cp{0.15\linewidth}cc}
\hline
\multicolumn{1}{c}{\textbf{Service}} & \multicolumn{1}{c}{\textbf{Function}}      & \multicolumn{1}{c}{\textbf{Tests (correct)}} & \multicolumn{1}{c}{\textbf{Tests (errors)}} \\ \hline
oauth2-token                         & OAuth2.0 token grant types                 & 3\tablefootnote{\label{tablefoot}Since OAuth flows are a multi-step process, same tests are reused in several business logic use cases}                                            & 12\textsuperscript{\ref{tablefoot}} \\
oauth2-code                          & OAuth2.0 code flows                        & 2\textsuperscript{\ref{tablefoot}}                                           & 9\textsuperscript{\ref{tablefoot}}                                         \\
oauth2-service                       & CRUD operations for Service entity         & 5                                            & 8                                           \\
oauth2-client                        & CRUD operations for Client entity          & 5                                            & 10                                          \\
oauth2-user                          & CRUD operations for User entity            & 6                                            & 11                                          \\
oauth2-refresh-token                 & CRUD operations on existing Refresh tokens & 3                                            & 3                                           \\
oauth2-key                           & Maintaining public key certificates        & 0                                            & 0                                           \\
mysqldb                              & Database storing all the data              & -                                            & -                                           \\ \hline
\end{tabular}

\end{table}
